Few-Shot Learning with Embedded Class Models and Shot-Free Meta Training

We propose a method for learning embeddings for few-shot learning that is suitable for use with any number of ways and any number of shots (shot-free). Rather than fixing the class prototypes to be the Euclidean average of sample embeddings, we allow them to live in a higher-dimensional space (embedded class models) and learn the prototypes along with the model parameters. The class representation function is defined implicitly, which allows us to deal with a variable number of shots per each class with a simple constant-size architecture. The class embedding encompasses metric learning, that facilitates adding new classes without crowding the class representation space. Despite being general and not tuned to the benchmark, our approach achieves state-of-the-art performance on the standard few-shot benchmark datasets.

==> plots_tables_dump.tex <==
\begin{table*}[htbp]
  \begin{center}
  \begin{tabular}{@{}c|c|c|c|c|c @{}}
    \hline
    Dataset & Testing Scenario & Training Scenario & As reported in \cite{Snell:nips17} & Our implementation of  \cite{Snell:nips17} & Our Method \\ 
        \hline
    \mi & \shot{1}{5} & \shot{1}{5} & 46.14 $\pm$ 0.77 & 43.88 $\pm$ 0.40 & 49.07 $\pm$ 0.43 \\ 
    \mi &  \shot{1}{5}&  \shot{1}{30} & 49.42 $\pm$ 0.78 & 48.36  $\pm$ 0.42 & 52.35  $\pm$ 0.40  \\ 
     \mi & \shot{5}{5} &  \shot{1}{5} & - & 58.33 $\pm$ 0.35 & 64.98 $\pm$ 0.35   \\ 
     \mi & \shot{5}{5} &  \shot{5}{5} &65.77 $\pm$ 0.70 & 65.49  $\pm$ 0.35 & 65.73 $\pm$ 0.36   \\ 
     \mi & \shot{5}{5} & \shot{5}{20} & 68.30 $\pm$ 0.66 & 68.29 $\pm$ 0.34 & 69.31 $\pm$ 0.33 \\ 
        \hline
            \hline
    \ti &\shot{1}{5} & \shot{1}{5}  & &41.36 $\pm$ 0.40 & 48.19 $\pm$ 0.43\\ 
    \ti & \shot {1}{5} & \shot{1}{30} & & 47.43 $\pm$ 0.45 & 53.90 $\pm$ 0.44\\ 
    \ti & \shot{5}{5} &  \shot{1}{5} & &55.93 $\pm$ 0.39 & 64.60 $\pm$ 0.39\\ 
    \ti & \shot{5}{5} &  \shot{5}{5} & &65.51 $\pm$ 0.38 & 65.50 $\pm$ 0.39\\ 
    \ti & \shot{5}{5} & \shot{5}{20} & &69.47 $\pm$ 0.38 & 71.15 $\pm$ 0.38\\ 
        \hline
             \hline
    \fs &\shot{1}{5} & \shot{1}{5}  & & 50.74 $\pm$ 0.48 & 55.14 $\pm$ 0.48\\ 
    \fs &\shot{1}{5} & \shot{1}{30} & &57.03 $\pm$ 0.50 & 60.68 $\pm$ 0.49\\ 
    \fs&\shot{5}{5} &  \shot{1}{5} & &64.63 $\pm$ 0.42 & 70.33 $\pm$ 0.40\\ 
    \fs&\shot{5}{5} &  \shot{5}{5} & &71.57 $\pm$ 0.38 & 71.66 $\pm$ 0.39\\ 
    \fs &\shot{5}{5} & \shot{5}{20} & &75.51 $\pm$ 0.37 & 75.69 $\pm$ 0.37\\ 
        \hline
                \hline
    \fc & \shot{1}{5} & \shot{1}{5}  & &36.09 $\pm$ 0.35 & 37.00 $\pm$ 0.35\\ 
    \fc & \shot{1}{5} & \shot{1}{30} & &37.10 $\pm$ 0.34 & 37.56 $\pm$ 0.33\\ 
    \fc & \shot{5}{5} &  \shot{1}{5} & &47.90 $\pm$ 0.35 & 49.38 $\pm$ 0.35\\ 
    \fc& \shot{5}{5} &  \shot{5}{5} & &49.62 $\pm$ 0.35 & 49.59 $\pm$ 0.35\\ 
    \fc& \shot{5}{5} & \shot{5}{20} & &50.44 $\pm$ 0.34 & 51.29 $\pm$ 0.37\\ 
        \hline
  \end{tabular}
  \end{center}
  \caption{Comparison of results from our method to that our implementation of \pn{} \cite{Snell:nips17} using the C64 network architecture.
  The table shows the accuracy and 95\% percentile confidence interval of our method on the \mi{} data set averaged over 2,000 episodes on different datasets.}
 \label{tab:baseline}
\end{table*}


paragraph{Relation to prototypical networks}
A closely related method to our approach is prototypical networks \cite{Snell:nips17}. This method uses episodic sampling but differs in the way the identify function is used. Here the episodes is split into a support set and a query set \ie $\mathcal E = \mathcal E_s \cup \mathcal E_q$. The identity function  is calculated as an arithmetic mean of the samples present in the support set. 
Given an episodes, the class means are calculated as 
\begin{equation}
c_n = \frac{1}{K_s} \sum_{j \in Y_k} \phi(x_j), x_j \in \mathcal E_s \cap  \mathcal{D}_{V_n}
\end{equation}
The samples in the query are then used to calculate the loss as described in \eqref{eq:proposed_loss}. We wish to point out that at meta-training, in addition to number of ways, the meta training also has the number of shots as a parameters. While the method only depends on the mean, the number of samples used to calculate the means affects the performance and this is shown empirically in the experiment section. We also show in the experiment section that our formulation leads to much better results in the $1$-shot scenario.

\paragraph{Relation to Center Loss}
Similar to our formulation, Center loss [] uses a mean that is learnt and also the Euclidean distance. However, this loss is usually used as a surrogate loss in  conjuction with a cross entropy classification loss. If the loss is used as the main loss, this will result in the collapse of the embedding. We explain why
\begin{equation}
 \mathcal {L}_{center} (\mathcal E) = \sum_{j=1}^{K_e} \sum_{n=1}^{N_f} y_j^i \|x_j^n - c_n\|^2
 \label{eq:center_loss}
\end{equation}
Now this loss function is convex. Hence, it can be solved in closed form. Calculating the gradients with respect to the paramters we get
\begin{align}
    \frac{\partial{ \mathcal {L}_{center} }}{\partial x_j^n} &= 2 (x_j^n - c_n) \\
    \frac{\partial{ \mathcal {L}_{center} }}{\partial c_n} &= -2 \sum_{j=1}^{K_e} (x_j^n - c_n)
\end{align}
Equating both gradient to zero and solving for the parameters results in $x_j^n = c_n$ and $c_n=\frac{1}{K_e} \sum_{j=1}^{K_e} x_j^n$. The global optimal solution is hence when all the points of a cluster have the same embedding, which leads to the embedding collapsing. 
}

